Isogeometric $C^1$ mortar method

We present an isogeometric mortar method for the discretization of the biharmonic equation posed on multi-patch domains. We assume only $C^0$-conformity at interfaces and employs a mortar approach to weakly enforce $C^1$-continuity across patch interfaces. Discrete inf-sup stability is ensured by selecting a Lagrange multiplier space consisting of splines of degree reduced by two compared to the primal space, with increased smoothness or merged elements near vertices. We prove optimal a priori error estimates and confirm the theoretical findings with a series of numerical experiments.

==> Iga_Mortar.tex <==
%\section{The isogeometric mortar formulation}\label{sec:iga_mortar_formulation}
%In this section we present the isogeometric discretization of the $C^1$ mortar formulation and analyze its convergence properties. 
\section{The isogeometric discretization}
We consider a standard $C^0$-conforming isogeometric multi-patch discretization. 
Each subdomain $\Omega_k$ is the image of the parametric space $\widehat{\Omega} = (0,1)^2$ by a spline geometry mapping $\bm{F}_k \colon \widehat{\Omega} \to \Omega_k$, with $\bm{F}_k \in {\Sp}^{\textbf{p}}_k \times {\Sp}^{\textbf{p}}_k$, satisfying the uniform regularity condition $\det \nabla \bm{F}_k \geq \gamma >0$ on $\H{\Omega}$. Here ${\Sp}^{\textbf{p}}_k = {\Sp}^{\textbf{p}}(\Xi^k_1,\Xi^k_2)$ is a spline space of fixed degree $\textbf{p}$ with (possibly different) quasi-uniform knot vectors in each direction.
Let us define the isogeometric discretization of the patch-local primal space on $\Omega_k$ as
\begin{equation}\label{eq:defXkh}
	X_{k,h}:=\Set{ v \in H^2(\Omega_k) : \; v \circ \bm{F}_{k} \in {\Sp}^{\textbf{p}}_{k} \mbox{ and }v = \dn v = 0 \mbox{ on } \partial\Omega\cap\partial\Omega_k}.
\end{equation}
We will define a global space under the assumption that the spaces are $C^0$-conforming. 
\begin{assumption}\label{ass:confmesh}
We assume that the multi-patch partition has no hanging nodes and that the meshes and spaces are {$C^0$-conforming}, that is for all $\ell \in \is$, the mesh that $\gl$ inherits from $\Omega_{m(\ell)}$ coincides with the one that it inherits from $\Omega_{s(\ell)}$.
Moreover, the trace spaces are equal, i.e., $X_{m(\ell),h} |_{{\Gamma}_\ell} = X_{s(\ell),h} |_{{\Gamma}_\ell}$.
\end{assumption}
We denote by $\mathcal{I}_{\mathcal{V},k}$ the set of indices of the four corners of the patch $\Omega_k$. The corners on the parameter domain $\widehat{\Omega}$ are denoted by $\widehat{\mathcal{V}}_{i,k} := \bm{F}_k^{-1}(\mathcal{V}_i)$, or with the more compact notation $\widehat{\mathcal{V}}_{i} \equiv \widehat{\mathcal{V}}_{i,k}$, when $k$ is fixed.

On $\Omega$ we define the space of isogeometric functions which are $C^0$ globally (i.e., in $H^1$) and $C^2$-continuous at the vertices of the decomposition
\begin{equation}\label{eq:spaceXh}
	X_h := \left\{v \in H^1(\Omega) : \;   v|_{\Omega_{k}} \in X_{k,h},\, \forall k \in \io, \text{ and } v \in C^2(\mathcal{V}_i), \, \forall i \in \iv \right\}.
\end{equation}
\begin{prop}
	We have $X_h \subset X$.
\end{prop}
\begin{proof}
Let $v\in X_h$. Since $\jump{\dn v}_{\gl} \in C^0(\gl)$, due to Assumption~\ref{ass:reg}, and $v \in C^2(\mathcal{V}_i), \, \forall i \in \iv$, $\jump{\dn v}_{\gl}$ is zero at the endpoints of $\gl$, then $\jump{\dn v}_{\gl} \in H^{1/2}_{00}(\gl)$, which yields $v \in X$.
\end{proof}
Furthermore, let $M_h := \prod_{\ell \in \is} M_\ell$ be a finite dimensional subspace of $M$, that will be defined later. We denote the mortar kernel as
\begin{equation}\label{eq:mortarkernel}
	V_h := \Set{v_h \in X_h : \; b(v_h, \mu_h) = 0, \quad \forall \mu_h \in M_h}.
\end{equation}
Thus, $V_h$ is the isogeometric space with weak $C^1$-continuity that depends on $M_h$. 
Now we are able to define the weak formulation of the model problem as a saddle point problem with $C^1$-mortar constraints along $\Sigma$: 
\textit{Find $(u_h, \lambda_h) \in X_h \times M_h$ such that}
\begin{equation}\label{eq:qh}
	\begin{cases}
		\begin{aligned}
			a(u_h, v_h) + b(v_h, \lambda_h)	 & = f(v_h) && \forall   v_h \in X_h \\
			b(u_h, \mu_h)	                 & = 0      && \forall \mu_h \in M_h.
		\end{aligned}
	\end{cases}
\end{equation}  

\subsection{Approximation properties of $X_h$}
\markboth{\MakeUppercase{Theoretical aspects}}{\MakeUppercase{Approximation properties of }$X_h$}

In what follows, we will denote by $C$ a positive, dimensionless constant, possibly different at each occurrence and independent of $h$.
\begin{remark}
If $s > 3$ the following Sobolev compact embedding holds, see~\cite[Theorem 6.2]{adams},
\begin{equation*}
	H^s(\widehat{\Omega}) \subset C^2\left(\overline{\widehat{\Omega}}\right).
\end{equation*}
\end{remark}
%\begin{definition}
Given an integer $s \geq 0$, the {bent Sobolev space} of order $s$, $\hh^s(\widehat{\Omega})$, is the space of functions that are in $H^s(Q)$ for all elements $Q$ of the mesh and have matching traces, up to $\min\{p-m, s-1 \}$ order derivatives, at the interelement interfaces, where $m$ is the multiplicity of the knot separating the two neighboring elements. The seminorms and norm of $\hh^s$ are defined as
\begin{equation*}
\begin{split}
	\abs{v}^2_{\hh^i(\widehat{\Omega})}  &:= \sum_{Q  \in \Q_h} \abs{v}^2_{H^i(Q)}, \quad 0 \leq i \leq s,\\
	\norm{v}^2_{\hh^s(\widehat{\Omega})} &:= \sum_{i = 0}^{s} \abs{v}^2_{\hh^i(\widehat{\Omega})}.
\end{split}
\end{equation*}
Bent Sobolev spaces on subdomains of $\widehat{\Omega}$, on $\Omega$, and its subspaces, are constructed in a similar way, see \cite{bazilevs} for more details.
%\end{definition}
\begin{prop}\label{prop:projparamdom}
Let $m$ and $t$ be integers such that $0 \leq t \leq m \leq p+1$ and let $s = \max (4,m)$. Then, there exists an operator 
%\footnote{\color{red}IF ALL THE PATCHES ARE PARAMETRIZED THE SAME, WHY DON'T WE DROP  $k$ FROM THE
%NOTATION OF  $ \widehat{\Pi}_{k,h} $? \GL{If we do not ask uniform meshes, the spline spaces could be different in each patch, right?}} 
$\widehat{\Pi}_{k,h} \colon \hh^4(\widehat{\Omega}) \to \H\Sp_{k}^{\mathbf{p}}$ such that
\begin{equation*}\label{eq:defproj}
	\widehat{\Pi}_{k,h} \widehat{v} = \widehat{v}, \quad \forall \, \widehat{v} \in \H\Sp_{k}^{\mathbf{p}}, \\
\end{equation*}
for all {$\iota \in \mathcal{I}_{\mathcal{V},k}$},
\begin{equation}\label{eq:projc2}
\begin{split}
	(\widehat{\Pi}_{k,h} \widehat{v})(\widehat{\mathcal{V}}_\iota) 		&=\widehat{v}(\widehat{\mathcal{V}}_\iota) \\
	\nabla (\widehat{\Pi}_{k,h} \widehat{v})(\widehat{\mathcal{V}}_\iota)	&=\nabla \widehat{v}(\widehat{\mathcal{V}}_\iota)\\
	\nabla (\nabla (\widehat{\Pi}_{k,h} \widehat{v}))(\widehat{\mathcal{V}}_\iota)	&= \nabla(\nabla \widehat{v})(\widehat{\mathcal{V}}_\iota),
\end{split}
\end{equation}
where $\nabla (\nabla)(\cdot)$ denotes the Hessian, and, for all $\widehat{v} \in \hh^s(\widehat{\Omega})$
\begin{equation}\label{eq:appproj}
	\norm*{\widehat{v} - \widehat{\Pi}_{k,h} \widehat{v}}_{\hh^t(\widehat{\Omega})} \leq C \, h^{m-t} \norm*{\widehat{v}}_{\hh^s(\widehat{\Omega})},
\end{equation}
and, for each edge $\H{\Gamma} \subset \partial \widehat{\Omega}$, we have 
\begin{equation}\label{eq:appprojbis}
	\norm{\nabla(\widehat{v} - \widehat{\Pi}_{k,h} \widehat{v})}_{L^2(\H{\Gamma})} + h\, \abs{\nabla(\widehat{v} - \widehat{\Pi}_{k,h} \widehat{v})}_{\hh^1(\H{\Gamma})} \leq C\,h^{m - \nicefrac{3}{2}} \norm{\widehat{v}}_{\hh^s(\widehat{\Omega})}.
\end{equation}
{\TT (This projector does not guarantee that the homogeneous b.c. on the domain boundary are satisfied. This is not completely trivial since there can be extraordinary vertices at the boundary.)}
\end{prop}
\begin{proof}
We consider the operator $\widetilde{\Pi}_h: H^1(0,1) \rightarrow \Sp^{p}(\Xi)$, as defined in~\cite[Equation 2.29]{beirao}, such that
\begin{equation}\label{eq:cappi}
	\widetilde{\Pi}_h(\widehat{v})(\hat{x}) = \sum_{j=1}^{n} \widetilde{\Lambda}_j(\widehat{v}) B_j(\hat{x}),
\end{equation}
where $n+p+1$ is the length of the knot vector $\Xi$, $\widehat{v}$ is a continuous function defined on the parametric interval $(0,1)$, $\widetilde{\Lambda}_j$ is a dual basis with $\widetilde{\Lambda}_1(\widehat{v}) = \widehat{v}(0)$, $\widetilde{\Lambda}_n(\widehat{v}) = \widehat{v}(1)$ and $\widetilde{\Lambda}_j(\widehat{v})$ for $2 \leq j \leq n-1$ is defined, {e.g.}, as in~\cite[Theorem 4.41]{schumaker}. By tensorization we can generalize~\eqref{eq:cappi} to the bivariate setting, obtaining $\widetilde{\Pi}_h: H^1(\widehat{\Omega}) \rightarrow \Sp^{p}(\Xi_1) \otimes \Sp^{p}(\Xi_2)$
\begin{equation}\label{eq:bivcappi}
	\widetilde{\Pi}_h(\widehat{v})(\hat{x}, \hat{y}) = \sum_{i=1}^{n_1}\sum_{j=1}^{n_2} \widetilde{\Lambda}_{(i,j)}(\widehat{v}) B_{(i,j)}(\hat{x}, \hat{y}),
\end{equation} 
where $\widetilde{\Lambda}_{(i,j)} = \widetilde{\Lambda}_{i} \otimes \widetilde{\Lambda}_{j}$. See Figure~\ref{fig:lambdabasis} for a visualization of the dual basis.
We recall that, from~\cite{schumaker, beirao} the following bounds hold:
\begin{align}\label{eq:lambdaprop}
	\abs{\widetilde{\Lambda}_{(i,j)} (\widehat{v})} &\leq Ch^{-1} \norm{\widehat{v}}_{L^2\left( \supp{B_{(i,j)}} \right) }, & (2,2) \leq (i,j) \leq (n_1,n_2)-(1,1), \notag \\
	\abs{\widetilde{\Lambda}_{(i,1)} (\widehat{v})} &\leq Ch^{-\nicefrac{1}{2}} \norm{\widehat{v}}_{L^2\left( (\supp{B_{i}})\times\{0\} \right) }, & 2 \leq i \leq n_1-1, \notag \\
	\abs{\widetilde{\Lambda}_{(i,n_2)} (\widehat{v})} &\leq Ch^{-\nicefrac{1}{2}} \norm{\widehat{v}}_{L^2\left( (\supp{B_{i}})\times\{1\} \right) }, & 2 \leq i \leq n_1-1, \\
	\abs{\widetilde{\Lambda}_{(1,j)} (\widehat{v})} &\leq Ch^{-\nicefrac{1}{2}} \norm{\widehat{v}}_{L^2\left( \{0\}\times(\supp{B_{j}}) \right) }, & 2 \leq j \leq n_2-1, \notag \\
	\abs{\widetilde{\Lambda}_{(n_1,j)} (\widehat{v})} &\leq Ch^{-\nicefrac{1}{2}} \norm{\widehat{v}}_{L^2\left( \{1\}\times(\supp{B_{j}}) \right) }, & 2 \leq j \leq n_2-1. \notag
\end{align}
Furthermore $\widetilde{\Pi}_h(\widehat{v})$ on each edge of $\partial \widehat{\Omega}$ only depends on $\widehat{v}$ on the given edge.

\input{Pictures/lambdabasis}

We modify the operator $\widetilde{\Pi}_h$ defined in~\eqref{eq:bivcappi} in order to fulfill~\eqref{eq:projc2}.
It is convenient to distinguish the degrees of freedom that are involved in the $C^2$ interpolation at the corners from the others on the boundary and the remaining ones in the interior of the patch. Hence we define
\begin{equation*}
	\ic := \Set{\textbf{i}=(i,j) \in \mathcal{I} \ | \ \exists \iota \in \mathcal{I}_{\mathcal{V},k}, \exists (\tilde{i},\tilde{j}) \mbox{ with } (0,0)\leq(\tilde{i},\tilde{j}),\mbox{ and }\tilde{i}+\tilde{j}\leq 2: \ \partial^{\tilde{i}}_{\hat{x}}\partial^{\tilde{j}}_{\hat{y}}B_{(i,j)}(\widehat{\mathcal{V}}_\iota)\neq 0}.
\end{equation*}
%Hence we indicate with $\ic$ the set of indices $\textbf{i}=(i,j)$ of the degrees of freedom that are depicted in blue in Figure~\ref{fig:referenceC2}, while $\iP$ is the whole set of indices. Moreover, $\iB$ stands for the set of indices of $\iP \setminus \ic$ that are depicted in green in Figure~\ref{fig:referenceC2}. \TT (here $\iB$ should be defined properly. It is a proper subset of $\iP \setminus \ic$!) \B \input{Pictures/referenceC2}
For all $(i,j) \in \mathcal{I} \setminus \ic$, $\Lambda_{(i,j)}$ is defined as
\begin{equation*}
	\Lambda_{(i,j)} := \widetilde{\Lambda}_{(i,j)}.
\end{equation*}
For all $(i,j) \in \ic$, the functionals $\Lambda_{(i,j)}$ have to be defined to fit the following constraints
\begin{align}
	\widehat{\Pi}_{k,h} \widehat{v}(\widehat{\mathcal{V}}_\iota) &= \widehat{v}(\widehat{\mathcal{V}}_\iota), & \partial_{\hat{x}\hat{x}} \widehat{\Pi}_{k,h} \widehat{v}(\widehat{\mathcal{V}}_\iota) &= \partial_{\hat{x}\hat{x}} \widehat{v}(\widehat{\mathcal{V}}_\iota) \notag\\
	\partial_{\hat{x}} \widehat{\Pi}_{k,h} \widehat{v}(\widehat{\mathcal{V}}_\iota) &= \partial_{\hat{x}} \widehat{v}(\widehat{\mathcal{V}}_\iota) & \partial_{\hat{x}\hat{y}} \widehat{\Pi}_{k,h} \widehat{v}(\widehat{\mathcal{V}}_\iota) &= \partial_{\hat{x}\hat{y}} \widehat{v}(\widehat{\mathcal{V}}_\iota) \label{eq:const}\\
	\partial_{\hat{y}} \widehat{\Pi}_{k,h} \widehat{v}(\widehat{\mathcal{V}}_\iota) &= \partial_{\hat{y}} \widehat{v}(\widehat{\mathcal{V}}_\iota) & \partial_{\hat{y}\hat{y}} \widehat{\Pi}_{k,h} \widehat{v}(\widehat{\mathcal{V}}_\iota) &= \partial_{\hat{y}\hat{y}} \widehat{v}(\widehat{\mathcal{V}}_\iota), \notag
\end{align}
for all $\iota \in \mathcal{I}_{\mathcal{V},k}$.
It is easy to see that~\eqref{eq:const} is a well posed interpolation problem that determines $\Lambda_{(i,j)}$ for all $(i,j) \in \ic$. In particular, for $\widehat{\mathcal{V}}_\iota = (0,0)$ and $\bigl\{ \Lambda_{(i,j)} \bigr\}_{i+j \leq 4}$, we obtain
\begin{equation*}
\begin{bmatrix}
	1 & 0 & 0 & 0 & 0 & 0 \\
	-1 & 1 & 0 & 0 & 0 & 0 \\
	-1 & 0 & 1 & 0 & 0 & 0 \\
	\frac{h_{1,1}+\theta_{1,2}}{h_{1,1}} & -\frac{2h_{1,1}+\theta_{1,2}}{h_{1,1}} & 0 & 1 & 0 & 0 \\
	1 & -1 & -1 & 0 & 1 & 0 \\
	\frac{h_{2,1}+\theta_{2,2}}{h_{2,1}} & 0 & -\frac{2h_{2,1}+\theta_{2,2}}{h_{2,1}} & 0 & 0 & 1
\end{bmatrix}
\begin{bmatrix}
	\Lambda_{(1,1)}\\
	\Lambda_{(2,1)}\\
	\Lambda_{(1,2)}\\
	\Lambda_{(3,1)}\\
	\Lambda_{(2,2)}\\
	\Lambda_{(1,3)}
\end{bmatrix}
	=
\begin{bmatrix}
	\widehat{v}(0,0)\\
	\frac{h_{1,1}}{p_1} \, \partial_{\hat{x}} \widehat{v}(0,0)\\
	\frac{h_{2,1}}{p_2} \, \partial_{\hat{y}} \widehat{v}(0,0)\\
	\frac{h_{1,1}(h_{1,1}+\theta_{1,2})}{p_1(p_1-1)} \, \partial_{\hat{x}\hat{x}} \widehat{v}(0,0)\\
	\frac{h_{1,1} h_{2,1}}{p_1 p_2} \, \partial_{\hat{x}\hat{y}} \widehat{v}(0,0)\\
	\frac{h_{2,1}(h_{2,1}+\theta_{2,2})}{p_2(p_2-1)} \, \partial_{\hat{y}\hat{y}} \widehat{v}(0,0)
\end{bmatrix},
\end{equation*}
where the coefficient matrix is non-singular, since it is lower-triangular. Note that here $\theta_{k,2}=h_{k,2}$ if the first knot in direction $k$ is a single knot, otherwise $\theta_{k,2}=0$. Thanks to Assumption~\ref{ass:quasiunif}, if $\widehat{v} \in \hh^4(\widehat{\Omega})$, we obtain
\begin{equation}\label{eq:1}
	\sum_{i+j \leq 4} \abs{\Lambda_{(i,j)}\widehat{v}} \leq C \left( \abs{\widehat{v}(0,0)} + h \norm{\nabla \widehat{v}(0,0)} +  h^2 \norm{\nabla(\nabla \widehat{v})(0,0)}\right),
\end{equation}
where $\norm{\cdot}$ denotes the vector or matrix norm and $C$ is independent of $h$. 
A similar bound holds for all $| \Lambda_{(i,j)} |$ with $(i,j) \in \ic$. Assume now that $Q \in \Q_h$ satisfies  $Q \subseteq \cup_{i + j \leq 4} \supp(B_{(i,j)})$, then we have
\begin{equation}\label{eq:11}
\begin{split}
	\norm{\widehat{\Pi}_{k,h}(\widehat{v})}_{L^2(Q)} &\leq \sum_{(i,j):\ Q \subseteq \supp(B_{(i,j)})} \abs{\Lambda_{(i,j)}\widehat{v}} \norm{B_{(i,j)}}_{L^2(Q)} \\
	&\leq C \sum_{\substack{(i,j):\ Q \subseteq \supp(B_{(i,j)}) \\ i+j > 4}} h \abs{\Lambda_{(i,j)}\widehat{v}} + C \sum_{ i+j \leq 4} h \abs{\Lambda_{(i,j)}\widehat{v}}.
\end{split}
\end{equation}
Then, from~\eqref{eq:lambdaprop}, \eqref{eq:1} and~\eqref{eq:11}, we conclude that
\begin{equation}\label{eq:12}
\begin{split}
	\norm{\widehat{\Pi}_{k,h} \widehat{v}}_{L^2(Q)} &\leq C 
	\left( \norm{\widehat{v}}_{L^2(\widetilde{Q})} + h^{\nicefrac{1}{2}} \norm{\widehat{v}}_{L^2\left( \partial \widetilde{Q} \cap \partial \widehat{\Omega} \right) } + h \abs{\widehat{v}(0,0)} + h^2 \norm{\nabla \widehat{v}(0,0)} + h^3 \norm{\nabla(\nabla \widehat{v})(0,0)}\right) \\
	&= C \opnorm{\widehat{v}}_{\widetilde{Q}},
\end{split}
\end{equation}
where $\widetilde{Q}$ is the {support extension} of $Q$, that is the union of the supports of basis functions whose support intersects $Q$, and $\opnorm{\cdot}_{\widetilde{Q}}$ is a short notation for the sum of norms appearing on the right-hand-side of~\eqref{eq:12}.
%\input{Pictures/reference00}
Let us consider a linear parametrization $T:[0,1]^2 \rightarrow \widetilde{Q}$ of $\widetilde{Q}$, i.e. $T([0,1]^2)=\widetilde{Q}$. Thanks to a scaling argument, it holds
\begin{equation}\label{eq:trace_scaling}
\begin{aligned}
	\norm{\widehat{v}}_{L^2\left( \partial \widetilde{Q} \cap \partial \widehat{\Omega} \right)} &\leq C h^{\nicefrac{1}{2}} \norm{\widehat{v} \circ T}_{L^2(T^{-1}(\partial \widetilde{Q} \cap \partial \widehat{\Omega}))} \leq C h^{\nicefrac{1}{2}} \norm{\widehat{v} \circ T}_{\hh^1([0,1]^2)} \\
	&= C h^{\nicefrac{1}{2}} \left( \norm{\widehat{v} \circ T}_{L^2([0,1]^2)} + \abs{\widehat{v} \circ T}_{H^1([0,1]^2)} \right) \leq C h^{\nicefrac{1}{2}} \left( h^{-1} \norm{\widehat{v}}_{L^2(\widetilde{Q})} +  \abs{\widehat{v}}_{\hh^1(\widetilde{Q})} \right) \\
	&= C \left( h^{-\nicefrac{1}{2}} \norm{\widehat{v}}_{L^2(\widetilde{Q})} + h^{\nicefrac{1}{2}} \abs{\widehat{v}}_{\hh^1(\widetilde{Q})} \right)%, \quad \forall \, \widehat{v} \in H^1(\widetilde{Q})
\end{aligned}
\end{equation}
and
\begin{equation*}
\begin{aligned}
	\abs{\widehat{v}(0,0)} &\leq \abs{\widehat{v}(T (0,0))} \leq C \left( \norm{\widehat{v} \circ T}_{L^2(T^{-1}(\partial \widetilde{Q} \cap \partial \widehat{\Omega}))} + \abs{\widehat{v} \circ T}_{\hh^1(T^{-1}(\partial \widetilde{Q} \cap \partial \widehat{\Omega}))} \right) \\
	&\leq C \left( \norm{\widehat{v} \circ T}_{L^2(T^{-1}(\widetilde{Q}))} + \abs{\widehat{v} \circ T}_{\hh^1(T^{-1}(\widetilde{Q}))} + \abs{\widehat{v} \circ T}_{\hh^2(T^{-1}(\widetilde{Q}))} \right) \\
	&\leq C \left( h^{-1}\norm{\widehat{v}}_{L^2(\widetilde{Q})} + \abs{\widehat{v}}_{\hh^1(\widetilde{Q})} + h \abs{\widehat{v}}_{\hh^2(\widetilde{Q})} \right)%, \quad \forall \, \widehat{v} \in H^2(\widetilde{Q}) 
\end{aligned}
\end{equation*}
Similarly, it also holds
\begin{equation*}
	\abs{\nabla \widehat{v}(0,0)} \leq C \left( h^{-1}\abs{\widehat{v}}_{\hh^1(\widetilde{Q})} + \abs{\widehat{v}}_{\hh^2(\widetilde{Q})} + h \abs{\widehat{v}}_{\hh^3(\widetilde{Q})} \right)
\end{equation*}
and
\begin{equation*}
	\abs{\nabla(\nabla \widehat{v})(0,0)} \leq C \left( h^{-1}\abs{\widehat{v}}_{\hh^2(\widetilde{Q})} + \abs{\widehat{v}}_{\hh^3(\widetilde{Q})} + h \abs{\widehat{v}}_{\hh^4(\widetilde{Q})} \right).
\end{equation*} 
In summary, we obtain
\begin{equation*}\label{eq:trinorm}
	\opnorm{\widehat{v}}_{\widetilde{Q}} \leq C \left( \norm{\widehat{v}}_{L^2(\widetilde{Q})} + h \norm{\widehat{v}}_{\hh^1(\widetilde{Q})} + h^2 \norm{\widehat{v}}_{\hh^2(\widetilde{Q})} + h^3 \norm{\widehat{v}}_{\hh^3(\widetilde{Q})} + h^4 \norm{\widehat{v}}_{\hh^4(\widetilde{Q})}  \right).
\end{equation*}
Following an argument like in~\cite[Lemma 3.1]{bazilevs}, we can prove that for any $\widehat{v} \in \hh^s (\widetilde{Q})$, there exists a spline $\widehat{w} \in \Sp^p_r$ such that
\begin{equation*}
	\opnorm{\widehat{v} - \widehat{w}}_{\widetilde{Q}} + h^t \abs{\widehat{v} - \widehat{w}}_{\hh^t (\widetilde{Q})} \leq C\,h^m \norm{\widehat{v}}_{\hh^s (\widetilde{Q})}. 
\end{equation*}
%\footnote{\color{red}(the argument above should be expanded and $p=2$ is a special case that should be written extra) \GL{not clear to me why}}
Combining the previous results and a standard inverse inequality, when $Q \subseteq \cup_{i + j \leq 4} \supp(B_{i,j})$
\begin{equation}\label{eq:hnorm}
\begin{split}
	\abs{\widehat{v} - \widehat{\Pi}_{k,h} \widehat{v}}_{\hh^t(Q)} &= \abs{\widehat{v} - \widehat{w} - \widehat{\Pi}_{k,h} (\widehat{v} - \widehat{w})}_{\hh^t(Q)} \\
	&\leq \abs{\widehat{v} - \widehat{w}}_{\hh^t(Q)} + C\,h^{-t} \norm{\widehat{\Pi}_{k,h} (\widehat{v} - \widehat{w})}_{L^2(Q)} \\
	&\leq \abs{\widehat{v} - \widehat{w}}_{\hh^t(Q)} + C\,h^{-t} \opnorm{\widehat{v} - \widehat{w}}_{\widetilde{Q}} \\
	&\leq C\,h^{m-t} \norm{\widehat{v}}_{\hh^s (\widetilde{Q})}.
\end{split}
\end{equation}
We remark that the same construction can be repeated for all $\widehat{\mathcal{V}}_\iota$, with $\iota \in \mathcal{I}_{\mathcal{V},k}$, and~\eqref{eq:hnorm} holds for $Q \nsubseteq \cup_{i + j \leq 4} \supp(B_{(i,j)})$, as proved in~\cite{bazilevs}. Finally~\eqref{eq:appproj} follows by summation over all mesh elements.\\
In order to prove~\eqref{eq:appprojbis} we proceed similarly. Given a mesh element $Q$ adjacent to the boundary $\partial \widehat{\Omega}$, let $E$ be one edge of $\partial Q$ on $\partial \widehat{\Omega}$.  Reasoning as in~\eqref{eq:trace_scaling} and thanks to~\eqref{eq:hnorm}, if we set $\eta := \widehat{v} - \widehat{\Pi}_{k,h} \widehat{v}$, we obtain  
\begin{equation*}
\begin{aligned}
	\norm{\nabla \eta}_{L^2(E)} &\leq C \left( h^{-\nicefrac{1}{2}} \norm{\nabla \eta}_{L^2(Q)} + h^{\nicefrac{1}{2}} \abs{\nabla \eta}_{H^1(Q)} \right) \\
	&\leq C \left( h^{-\nicefrac{1}{2}} \abs{\eta}_{H^1(Q)} + h^{\nicefrac{1}{2}} \abs{\eta}_{H^2(Q)} \right) \\
	&\leq C h^{m-\nicefrac{3}{2}} \norm{\widehat{v}}_{\hh^s(\widetilde{Q})}
\end{aligned}
\end{equation*}
and
\begin{equation*}
\begin{aligned}
	\norm{\nabla \eta}_{H^1(E)} &\leq C \left( h^{-\nicefrac{1}{2}} \abs{\nabla \eta}_{H^1(Q)} + h^{\nicefrac{1}{2}} \abs{\nabla \eta}_{H^2(Q)} \right) \\
	&\leq C \left( h^{-\nicefrac{1}{2}} \abs{\eta}_{H^2(Q)} + h^{\nicefrac{1}{2}} \abs{\eta}_{H^3(Q)} \right) \\
	&\leq C h^{m-\nicefrac{5}{2}} \norm{\widehat{v}}_{\hh^s(\widetilde{Q})}.
\end{aligned}
\end{equation*}
Then~\eqref{eq:appprojbis} follows. Note also that $\nabla \widehat{v} -  \nabla \widehat{\Pi}_{k,h} \widehat{v} \in H^1_0(\H{\Gamma})$ for each edge $\H{\Gamma}$ of $\partial \widehat{\Omega}$. Indeed $\nabla \widehat{v}$ is interpolated at the vertices, that is $\nabla \widehat{v} -  \nabla \widehat{\Pi}_{k,h} \widehat{v}$ vanishes at the endpoints of $\H{\Gamma}$.
\end{proof}
With homogeneous boundary conditions, we have \eqref{eq:appprojbis}
under weaker regularity, as stated below.
\begin{prop}\label{prop:projparamdom_low-H2_regularity}
Let $\Gamma$ be an edge of $\Omega_k$ and $\widehat{\Gamma}$ its pre-image, (an edge of $ \widehat{\Omega}$). There exists an operator 
\begin{equation*}
	\widehat{\Pi}^0_{k,h} \colon
	\left \{\widehat{ v} \in \hh^2( \widehat{\Omega}) \cap H^1_0( \widehat{\Omega}) :\; \nabla \widehat{v}|_{\widehat{\Omega} \setminus {\widehat{\Gamma}}} = 0 \right \} \to \left \{\widehat{v}\in \H\Sp^{p}(\Xi) \cap H^1_0( \widehat{\Omega}) :\; \nabla \widehat{v}|_{\widehat{\Omega} \setminus {\widehat{\Gamma}}} = 0 \right \}
\end{equation*}
such that
\begin{equation*}%\label{eq:appprojbis}
	\norm{\nabla(\widehat{v} - \widehat{\Pi}^0_{k,h} \widehat{v})}_{L^2(\H{\Gamma})} + h\, \abs{\nabla(\widehat{v} - \widehat{\Pi}^0_{k,h} \widehat{v})}_{\hh^1(\H{\Gamma})} \leq C\,h^{\nicefrac{1}{2}} \norm{\widehat{v}}_{\hh^2(\widehat{\Omega})}.
\end{equation*}
Here $\H\Sp^{p}(\Xi)$ is the trace space of $\H\Sp^{\mathbf{p}}_k$ corresponding to the edge $\widehat{\Gamma}$.
\end{prop}
\begin{proof}
The operator $\widehat{\Pi}^0_{k,h} $ is as
$\widehat{\Pi}_{k,h} $ in Proposition \ref{prop:projparamdom} where
only interior dual basis functions are active, see Figure~\ref{fig:lambdabasis}. This
is similar to \cite[Lemma 3.6]{bazilevs}. 
\end{proof}
\begin{prop}\label{prop:projsplinec2}
Let $m$ and $t$ be integers such that $0 \leq t \leq m \leq p+1$ and let $s = \max (4,m)$.
Then, there exists an operator $\Pi_{k,h} \colon H^4(\Omega_k) \cap H^2_*(\Omega_k) \to X_{k,h}$ such that
\begin{equation*}
	\Pi_{k,h} v = v, \quad \forall v \in X_{k,h}, \\
\end{equation*}
with
\begin{equation}\label{eq:c2phys}
\begin{split}
	(\Pi_{k,h} v)(\mathcal{V}_\iota) 		&=  v(\mathcal{V}_\iota) \\
	\nabla (\Pi_{k,h} v)(\mathcal{V}_\iota)	&=\nabla v(\mathcal{V}_\iota)\\
	\nabla(\nabla (\Pi_{k,h} v))(\mathcal{V}_\iota)	&= \nabla(\nabla v)(\mathcal{V}_\iota),
\end{split}
\end{equation}
for all $\iota \in \mathcal{I}_{\mathcal{V},k}$, and
\begin{equation}\label{eq:physapp}
	\norm*{v - \Pi_{k,h} v}_{\hh^t(\Omega_k)} \leq C \, h^{m-t} \norm*{v}_{\hh^s(\Omega_k)}.
\end{equation}
Moreover, for each edge $\Gamma$ of $\partial \Omega_k \setminus \partial\Omega$, we have
\begin{equation}\label{eq:physappbis}
	\norm{\nabla(v - \Pi_{k,h} v)}_{L^2(\Gamma)} + h\, \abs{\nabla(v - \Pi_{k,h} v)}_{\hh^1(\Gamma)} \leq C\, h^{m - \nicefrac{3}{2}} \norm{v}_{\hh^s(\Omega_k)}.
\end{equation}
{\TT (I removed the definition of $H^2_*(\Omega_k)$, so we should also remove/replace it here. Moreover, just restricting the domain to functions that satisfy the homogeneous global b.c. does not guarantee the b.c. for the projection! I would propose to define the projector for $H^4(\Omega_k)$ and then state the additional condition:)\\
Moreover, for each boundary edge $\Gamma \subset \partial \Omega$ we have
\[
 \Pi_{k,h} v|_\Gamma = \dn \Pi_{k,h} v|_\Gamma = 0.
\]
(proof needs to be fixed as well)
}
\end{prop}
\begin{proof}
We define the projector $\Pi_{k,h} \colon H^4(\Omega_k)\cap H^2_*(\Omega_k) \to X_{k,h}$ as
\begin{equation*}
	\Pi_{k,h} v := (\widehat{\Pi}_{k,h}(v \circ \bm{F}_k)) \circ \bm{F}_k^{-1}, \quad \forall \, v \in H^4(\Omega_k)\cap H^2_*(\Omega_k),
\end{equation*}
where $\widehat{\Pi}_{k,h}$ is defined in Proposition~\ref{prop:projparamdom}.
Then, \eqref{eq:c2phys} follows from \eqref{eq:const} and the chain rule. Also \eqref{eq:physapp}-\eqref{eq:physappbis} follow from the chain rule, see \cite[Section 3]{bazilevs} for more details.
\end{proof}
We can now define a projector onto $X_h$ by a patchwise construction.
\begin{prop}\label{prop:globalproj} 
Let $m$ be an integer such that $0 \leq m \leq p+1$ and let $s = \max (4,m)$. There exists a multi-patch operator $\Pi_h \colon H^4(\Omega) \cap H^2_0(\Omega) \to X_h$ such that
\begin{equation*}
	\norm{v - \Pi_h v}_X \leq C\,h^{m-2}\,\norm{v}_{H^s(\Omega)}.
\end{equation*}
\end{prop}
\begin{proof}
Let $v$ be in $H^4(\Omega) \cap H^2_0(\Omega)$. We define $\Pi_h$ as
\begin{equation*}
	(\Pi_h v)|_{\Omega_k} = \Pi_{k,h} (v|_{\Omega_k}), \quad \forall k \in \io.
\end{equation*}
The norm $\norm{\cdot}_X$ consists of patchwise $H^2$-norm contributions and norms of jumps of normal derivatives across all interfaces. The bounds for the $H^2$-norms follow from Proposition~\ref{prop:projsplinec2} with $t=2$. What remains is to prove that, for all $\ell \in \is$,
\begin{equation*}
	\norm{\jump{\dn v - \dn \Pi_h v}}_{H^{\nicefrac{1}{2}}(\gl)} \leq C\,h^{m-2}\,\norm{v}_{H^s\left( \Omega_{m(\ell)} \cup \Omega_{s(\ell)}\right) }.
\end{equation*}
From~\eqref{eq:physappbis}, it holds
\begin{align*}
	\norm{(\nabla v - \nabla \Pi_h v)|_{\Omega_{s(\ell)}}}_{L^2(\gl)} &\leq C\,h^{m-\nicefrac{3}{2}}  \norm{v}_{H^s\left( \Omega_{s(\ell)}\right) }, \\
	\norm{(\nabla v - \nabla \Pi_h v)|_{\Omega_{s(\ell)}}}_{H^1(\gl)} &\leq C\,h^{m-\nicefrac{5}{2}} \norm{v}_{H^s\left( \Omega_{s(\ell)}\right)}.
\end{align*}
Interpolating between $L^2(\gl)$ and $H^1(\gl)$, we get
\begin{equation*}
	\norm{(\nabla v - \nabla \Pi_h v)|_{\Omega_{s(\ell)}}}_{H^{\nicefrac{1}{2}}(\gl)} \leq C\,h^{m-2} \abs{v}_{H^s\left( \Omega_{s(\ell)}\right) }.
\end{equation*}
Similarly, we also obtain
\begin{equation*}
	\norm{(\nabla v - \nabla \Pi_h v)|_{\Omega_{m(\ell)}}}_{H^{\nicefrac{1}{2}}(\gl)} \leq C\,h^{m-2} \abs{v}_{H^s\left( \Omega_{m(\ell)}\right) }.
\end{equation*}
Finally, it holds
\begin{align*}
	\norm{\jump{\dn v - \dn \Pi_h v}}_{H^{\nicefrac{1}{2}}(\gl)} &\leq \norm{(\nabla v - \nabla \Pi_h v)|_{\Omega_{s(\ell)}}}_{H^{\nicefrac{1}{2}}(\gl)} + \norm{(\nabla v - \nabla \Pi_h v)|_{\Omega_{m(\ell)}}}_{H^{\nicefrac{1}{2}}(\gl)}\\
	& \leq  C\,h^{m-2}\,\norm{v}_{H^s\left( \Omega_{m(\ell)} \cup \Omega_{s(\ell)}\right), }
\end{align*}
which concludes the proof.
\end{proof}

%\begin{remark}\label{rem:globalproj}
%Thanks to the properties of $\Pi_{k,h}$, we can construct the multi-patch interpolant
%\begin{equation}
%(s_h v)|_{\Omega_k} = \Pi_{k,h} (v|_{\Omega_k}), \quad \forall k \in \io.
%\end{equation}
%From~\cite[Proposition 3.8]{beirao}, follows that $s_h$ is a projector from $C^0(\overline{\Omega})$ to $X_h$.
%\end{remark}

\subsection[Approximation properties of $V_h$]{Approximation properties of $V_h$}
\markboth{\MakeUppercase{Theoretical aspects}}{\MakeUppercase{Approximation properties of }$V_h$}
The aim of this section is to prove the estimate
\begin{equation*}
	\inf_{v_h \in V_h} \norm{u - v_h}_X \leq C h^{p - 1} \norm{u}_{H^{s}(\Omega)},
\end{equation*}
where $s = \max (4,p+1)$ and $\norm{\cdot}_X$ is the norm defined in~\eqref{eq:normX}. We recall that $V_h$ depends on the choice of $M_h$, on which we ask the following general assumption.
\begin{assumption}\label{ass:oderM}
	For every $\ell \in \is$ and for any $\tau \in H^{p - \nicefrac{3}{2}}(\gl)$, it holds
	\begin{equation*}
		\inf_{\mu_h \in M_\ell} \norm{\tau - \mu_h}_{L^2(\gl)} \leq C h^{p - \nicefrac{3}{2}} \norm{\tau}_{H^{p - \nicefrac{3}{2}}(\gl)}.
	\end{equation*}
\end{assumption}
{\color{red}We assume to have given a discrete multiplier space which, on the one hand, satisfies certain approximation properties and, on the other hand, has the same dimenison as the discrete trace space and satisfies an inf-sup condition as specified in Assumption~\ref{ass:dim_infsup}}. We introduce the discrete trace derivative space $W_h$ defined as $W_h := \prod_{\ell \in \is} W_{\ell}$, where
\begin{equation}\label{eq:defWl}
	W_{\ell} := \left\{w \in L^2(\gl) : \; w = \dn v_h |_{\gl}, \mbox{ with }\quad
	\begin{aligned} 
	& v_h \in X_{s(\ell),h} \cap H^1_0\left( \Omega_{s(\ell)}\right), \\
	& \nabla(\nabla v_h)(\mathcal{V}_\iota) = 0^{2\times 2}, \mbox{ for all }\iota \in \mathcal{I}_{\mathcal{V},s(\ell)} \\
	& {\TT \mbox{(or:) }\dn \partial_{\tau} v_h(\mathcal{V}_\iota) = 0, \mbox{ for all }\iota \in \mathcal{I}_{\mathcal{V},s(\ell)}} \\
	& {\TT \mbox{(or old version:) }\dn v_h|_{\partial \Omega_{s(\ell)} \setminus {\Gamma}_{\ell}} = 0}
	\end{aligned}\right\}.
\end{equation}
\begin{remark}
Functions in $W_{\ell}$ are zero with zero derivative at the endpoints of the interface $\gl$.
\end{remark}
\begin{remark}\label{rem:dofs}
Observe that the degrees-of-freedom (control points) that are relevant for $W_\ell$ are not involved in $W_{\ell'}$, $\ell' \neq \ell$. In Figure~\ref{fig:dofs} the degrees of freedom associated to the $C^2$-constraints on the vertices are marked in red, the ones associated with the $C^0$-constraints along the interfaces are marked in blue, while the degrees of freedom of $v_h$ such that $\partial_n v_h$ spans $W_\ell$ are depicted in green.
\end{remark}
\input{Pictures/dofs2}
\begin{prop}\label{prop:orderW-H12}
For each $w \in H_{00}^{\nicefrac{1}{2}}(\gl)$, it holds
\begin{equation}\label{eq:orderW-H12}
	\inf_{w_h \in W_{\ell}} \norm{w - w_h}_{L^2(\gl)} \leq C \, h^{\nicefrac{1}{2}} \, \norm{w}_{H^{\nicefrac{1}{2}}(\gl)}.
\end{equation}
\end{prop}
\begin{proof}
Let  $w \in H_{00}^{\nicefrac{1}{2}}(\gl)$, then the solution $v$ of
\begin{equation*}
\begin{cases}
	\begin{aligned}
		\Delta^2v &= 0 && \text{in }\Omega_{s(\ell)} \\
		v &= 0 && \text{on }\partial \Omega_{s(\ell)} \\
		\partial_n  v &= w && \text{on }  {\Gamma}_{\ell}\\
		\partial_n  v&= 0 && \text{on }\partial \Omega_{s(\ell)} \setminus {\Gamma}_{\ell}
	\end{aligned}
\end{cases}
\end{equation*}
fulfils  $v \in H^2(\Omega_{s(\ell)}) \cap H^1_0(\Omega_{s(\ell)})$
and $\norm{v}_{H^2(\Omega_{s(\ell)})} \leq C \norm{w}_{H_{00}^{\nicefrac{1}{2}}(\gl)}$. 
Thanks to  Proposition \ref{prop:projparamdom_low-H2_regularity}, we can define a projector
\begin{equation*}\small
	\Pi^{0}_{s(\ell),h}: \Set{v_h \in X_{s(\ell),h} \cap
		H^1_0(\Omega_{s(\ell)}) \ | \ \partial_{n}v_h|_{\partial
			\Omega_{s(\ell)} \setminus \mathring{\Gamma}_{\ell}} = 0}
	\rightarrow \Set{v_h \in X_{s(\ell),h} \cap H^1_0(\Omega_{s(\ell)}) \
		| \ \partial_{n}v_h|_{\partial \Omega_{s(\ell)} \setminus
			\mathring{\Gamma}_{\ell}} = 0}
\end{equation*}
such that
\begin{equation*}\label{eq:est_trace1}
	\norm{\nabla(v - \Pi^{0}_{s(\ell),h} v)}_{L^2(\gl)} \leq C\, h^{\nicefrac{1}{2}} \norm{v}_{\hh^2(\Omega_{s(\ell)})}.	
\end{equation*}
Thus, we can define a projector $P_{h,\ell}:H_{00}^{\nicefrac{1}{2}}(\gl) \rightarrow W_{\ell}$ as $P_{h,\ell}(w):= (\dn \Pi^{0}_{s(\ell),h} v)|_{\gl}$.\\
Finally, it holds that
\begin{align*}
	\norm{w - P_{h,\ell}w}_{L^2(\gl)} & \leq \norm{\nabla (v - \Pi^{0}_{s(\ell),h} v)}_{L^2(\gl)} \leq Ch^{\nicefrac{1}{2}} \abs{v}_{H^2(\Omega_{s(\ell)})} \\
	&\leq Ch^{\nicefrac{1}{2}} \norm{w}_{H^{\nicefrac{1}{2}}(\gl)},
\end{align*}
which is the desired statement.
\end{proof}
We define the mortar projection $\M_h$ by
\begin{equation*}
	(\M_h v)|_{\gl} := \M_{\ell}(v|_{\gl}), \quad \forall v \in L^2(\Sigma),
\end{equation*}
where, for every $\ell \in \is$, the local projection $\M_\ell \colon L^2(\gl) \to W_\ell$ is defined as
\begin{equation*}\label{eq:mortarproj}
	\int_{\gl} \M_\ell v \, \mu \, d\sigma = \int_{\gl} v \, \mu \, d\sigma, \quad \forall \mu \in M_{\ell}.
\end{equation*}
In order to guarantee the well-posedness of the mortar projection the following assumption is introduced.
\begin{assumption}\label{ass:dim_infsup}
For every $\ell \in \is$ the discrete trace space $W_\ell$ and the discrete multiplier space $M_\ell$ have the same dimension, {i.e.}, $\dim(W_\ell) = \dim(M_\ell)$, and there exists a constant $\beta_\ell > 0$ independent of $h$ such that
\begin{equation*}
	\sup_{w_h \in W_\ell} \dfrac{\int_{\gl} w_h \, \mu_h d\sigma}{\norm{w_h}_{L^2(\gl)}} \geq \beta_\ell \norm{\mu_h}_{L^2(\gl)}, \quad \forall \mu_h \in M_\ell.
\end{equation*}
\end{assumption}
\begin{remark}\label{rem:bothstab}
Given Assumption~\ref{ass:dim_infsup}, it follows from~\cite[Proposition 3.4.3]{boffi} that, for every $\ell \in \is$, it holds
\begin{equation*}
	\sup_{\mu_h \in M_\ell} \dfrac{\int_{\gl} w_h \, \mu_h d\sigma}{\norm{\mu_h}_{L^2(\gl)}} \geq \beta_\ell \norm{w_h}_{L^2(\gl)}, \quad \forall w_h \in W_\ell .
\end{equation*}
\end{remark}
\begin{corollary}\label{cor:pistablel2}
For every $\ell \in \is$ the mortar projection $\M_\ell \colon L^2(\gl) \to W_\ell$ is well defined and $L^2$-stable.
\end{corollary}
\begin{proof}
From Assumptions~\ref{ass:dim_infsup} and from \cite[Proposition 3.4.3]{boffi} the matrix $B$ associated with the scalar product $(w,\mu)_{L^2}$ on $W_{\ell} \times M_{\ell}$ is square and invertible, so $\M_\ell$ is well defined. Moreover, from \cite[Theorem 4.2.3]{boffi} it follows that $\M_{\ell}$ is $L^2$-stable.
\end{proof}
%\begin{corollary}\label{cor:pistableh1}
%	Given Assumption~\ref{ass:dim_infsup}, for every $\ell \in \ig$ the mortar projection $\M_\ell$ is $H^{\nicefrac{1}{2}}_{00}$-stable.
%\end{corollary}
%\begin{proof}\color{red}
%	%\TT (I don't get this proof.) \B
%	Let $w \in H^1_{00}(\gl)$ and let $P_{h,\ell}$ be the spline approximation operator as in the proof of Proposition~\ref{prop:orderW-H12}. Using the inverse inequality for splines, we obtain
%	\begin{equation*}
%		\begin{split}
%			\norm{\M_\ell \, w}_{H^{\nicefrac{1}{2}}(\gl)} &\leq \norm{\M_\ell \, w - P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)} + \norm{P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)} \\
%			&= \norm{\M_\ell (w - P_{h,\ell} w)}_{H^{\nicefrac{1}{2}}(\gl)} + \norm{P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)} \\
%			&\leq C h^{-\nicefrac{1}{2}} \norm{\M_\ell (w - P_{h,\ell} w)}_{L^2(\gl)} + \norm{P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)},
%		\end{split}
%	\end{equation*}
%	but from Corollary~\ref{cor:pistablel2} and the approximation properties of $P_{h,\ell}$, it follows
%	\begin{equation*}
%		\begin{split}
%			\norm{\M_\ell \, w}_{H^{\nicefrac{1}{2}}(\gl)} &\leq C h^{-\nicefrac{1}{2}} \norm{w - P_{h,\ell} w}_{L^2(\gl)} + \norm{P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)} \\
%			&\leq C \norm{w}_{H^{\nicefrac{1}{2}}(\gl)} + \norm{P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)}.
%		\end{split}
%	\end{equation*}
%%	Interpolating~\eqref{eq:est_trace1} between $L^2$ and $H^1$ we get
%%	\begin{equation*}
%%		\norm{P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)} \leq \norm{w}_{H^{\nicefrac{1}{2}}(\gl)} + \norm{w - P_{h,\ell} w}_{H^{\nicefrac{1}{2}}(\gl)} \leq C \norm{w}_{H^{\nicefrac{1}{2}}(\gl)}
%%	\end{equation*}
%%	 and then the thesis follows.
%\end{proof}
\begin{lemma}\label{lemma:projproperties}
There exists a constant $C > 0$ such that, for every $\ell \in \is$ and for every $w \in H^{\nicefrac{1}{2}}_{00}(\gl)$, 
\begin{equation*}
	\norm{w - \M_\ell \, w}_{L^2(\gl)} \leq C \,h^{\nicefrac{1}{2}}\norm{w}_{H^{\nicefrac{1}{2}}(\gl)}.
\end{equation*}
Furthermore, the mortar projection $\M_\ell$ is $H^{\nicefrac{1}{2}}_{00}$-stable.
\end{lemma}
\begin{proof}
Let $w \in H^1_{00}(\gl)$ and let $P_{h,\ell}$ be the spline approximation operator as in the proof of Proposition~\ref{prop:orderW-H12}. It holds
\begin{equation}\label{eq:mortar_est}
\begin{split}
	\norm{w - \M_\ell \, w}_{L^2(\gl)} &\leq \norm{w - P_{h,\ell} w - \M_\ell (w - P_{h,\ell} w)}_{L^2(\gl)} \\
	&\leq C \norm{w - P_{h,\ell} w}_{L^2(\gl)} \leq C \, h^{\nicefrac{1}{2}} \norm{w}_{H^{\nicefrac{1}{2}}(\gl)}.
\end{split}
\end{equation}
For what concerns the $H^{\nicefrac{1}{2}}_{00}$-stability, using the inverse inequality for splines and~\eqref{eq:mortar_est}, we have
\begin{align*}
	\norm{\M_\ell \, w}_{H^{\nicefrac{1}{2}}(\gl)} &\leq \norm{w}_{H^{\nicefrac{1}{2}}(\gl)} + \norm{w - \M_\ell \, w}_{H^{\nicefrac{1}{2}}(\gl)} \leq \norm{w}_{H^{\nicefrac{1}{2}}(\gl)} + C h^{-\nicefrac{1}{2}}\norm{w - \M_\ell \, w}_{L^2(\gl)} \\
	&\leq C \norm{w}_{H^{\nicefrac{1}{2}}(\gl)},
\end{align*}
which completes the proof.
\end{proof}
In addition to the local projector $\M_\ell$, for every $\ell \in \is$, we introduce the {dual} operator $\M_{\ell}^{*} \colon L^2(\gl) \to M_\ell$ by
\begin{equation}\label{eq:mortarprojdual}
	\int_{\gl} \M_{\ell}^{*} \mu \, v \, d\sigma = \int_{\gl} \mu \, v \, d\sigma, \quad \forall v \in W_{\ell}.
\end{equation}
\begin{lemma}\label{lemma:dualproperties}
For every $\ell \in \is$, the dual operator $\M_{\ell}^{*} \colon L^2(\gl) \to M_\ell$ is well-defined and $L^2$-stable. Furthermore, there exists a constant $C > 0$ such that, for all $\mu \in H^{p - \nicefrac{3}{2}}(\gl)$, it holds
\begin{equation}
	\norm{\mu - \M_{\ell}^{*} \, \mu}_{L^2(\gl)} \leq C\,h^{p - \nicefrac{3}{2}}\, \norm{\mu}_{H^{p - \nicefrac{3}{2}}(\gl)}.
\end{equation}
\end{lemma}
\begin{proof}
As in the proof of Corollary~\ref{cor:pistablel2}, Assumption~\ref{ass:dim_infsup} guarantees that $\M_{\ell}^{*}$ is well-defined. Combining Assumption~\ref{ass:dim_infsup} with~\eqref{eq:mortarprojdual}, we get
\begin{equation*}
\begin{split}
	\norm{\M_{\ell}^{*}\,\mu}_{L^2(\gl)} &\leq \frac{1}{\beta_\ell} \sup_{w_h \in W_{\ell}}\frac{\int_{\gl}\M_{\ell}^{*}\,\mu \, w_h\,d\sigma}{\norm{w_h}_{L^2(\gl)}} \\
	&= \frac{1}{\beta_\ell} \sup_{w_h \in W_{\ell}}\frac{\int_{\gl}\mu \, w_h\,d\sigma}{\norm{w_h}_{L^2(\gl)}} \\
	&\leq \frac{1}{\beta_\ell} \sup_{w_h \in W_{\ell}} \frac{\norm{\mu}_{L^2(\gl)} \norm{w_h}_{L^2(\gl)}}{\norm{w_h}_{L^2(\gl)}} = \frac{1}{\beta_\ell} \norm{\mu}_{L^2(\gl)}.
\end{split}
\end{equation*}
The approximation property of $\M_{\ell}^{*}$ follows from Assumption~\ref{ass:oderM}. Indeed, for  $\mu \in H^{p - \nicefrac{3}{2}}(\gl)$, let $\mu_h \in M_\ell$ be such that 
\begin{equation*}
	\norm{\mu - \mu_h}_{L^2(\gl)} \leq C h^{p - \nicefrac{3}{2}} \norm{\mu}_{H^{p - \nicefrac{3}{2}}(\gl)},
\end{equation*} 
then  
\begin{equation*}
\begin{split}
	\norm{\mu - \M_{\ell}^{*} \mu}_{L^2(\gl)} &= \norm{\mu - \mu_h - \M_{\ell}^{*}(\mu - \mu_h)}_{L^2(\gl)} \\
	&\leq C' \norm{\mu - \mu_h}_{L^2(\gl)} \leq C\,h^{p - \nicefrac{3}{2}}\, \norm{\mu}_{H^{p - \nicefrac{3}{2}}(\gl)},
\end{split}
\end{equation*}
which completes the proof.
\end{proof}
We can now address the study of the properties of $V_h$.
\begin{lemma}\label{lemma:eqbrokennorm2}
There exists a constant $C > 0$, independent of $h$, such that, for every $v_h \in V_h$, it holds
\begin{equation*}
	\sum_{k \in \io} \norm{v_h}^2_{H^2(\Omega_k)} \leq C\sum_{k \in \io} \abs{v_h}^2_{H^2(\Omega_k)}.
\end{equation*}
\begin{proof}
The proof follows the lines of~\cite[Theorem 1]{marcinkowski}. We first demonstrate that for all $v_h \in V_h$ it holds
\begin{equation}\label{eq:est1}
	\sum_{k \in \io} \norm{\partial_x v_h}^2_{L^2(\Omega_k)} \leq C\sum_{k \in \io} \abs{v_h}^2_{H^2(\Omega_k)}.
\end{equation}
For any $(x,y) \in \Omega$, let $(a,y),(b,y) \in \partial \Omega$ be the endpoints of a segment that contains $(x,y)$ and let us define
\begin{equation*}
	I[a,x]:= \Set{t \in [a,x] | (t, y) \in \Gamma},
\end{equation*}
and $N_I= |I[a,b]|$. Then
\begin{equation}\label{eq:est2}
	\partial_x v_h(x,y) = \int_a^x \partial_{xx} v_h(t,y) \, dt + \sum_{t_{\ell} \in I[a,x]}\jump{\partial_x v_h}_{\gl}(t_{\ell},y).
\end{equation}
The first term in the right-hand side of~\eqref{eq:est2} is bounded by
\begin{equation*}
	\abs*{\int_a^x \partial_{xx} v_h(t,y) \, dt} \leq \int_a^b \abs*{\partial_{xx} v_h(t,y)}\, dt
	\leq M^{\nicefrac{1}{2}} \left( \int_a^b \abs*{\partial_{xx} v_h(t,y)}^2dt\right)^{\nicefrac{1}{2}},
\end{equation*}
where $M=\mbox{diam}(\Omega)$, while the second term is bounded by
\begin{equation*}
\begin{split}
	\abs*{\sum_{t_{\ell} \in I[a,x]}\jump{\partial_x v_h}_{\gl}(t_{\ell},y)} &\leq \sum_{t_{\ell} \in I[a,b]}\abs*{\jump{\partial_x v_h}_{\gl}(t_{\ell},y)}\\
	&\leq \left( N_I \right)^{\nicefrac{1}{2}} \left( \sum_{t_\ell \in I[a,b]} \abs*{\jump{\partial_x v_h}(t_\ell,y)}^2 \right)^{\nicefrac{1}{2}}.
\end{split}
\end{equation*}
Hence we obtain
\begin{equation}\label{eq:aux01}
	\abs*{\partial_x v_h(x,y)}^2 \leq C \int_a^b \abs*{\partial_{xx} v_h(t,y)}^2 \, dt + C \sum_{t_\ell \in I[a,b]} \abs*{\jump{\partial_x v_h}_{\gl}(t_\ell,y)}^2.
\end{equation}
Assume w.l.o.g. that $\Omega \subset \left[ 0,  M \right] ^2$ and that $\abs*{\partial_{xx} v_h(t,y)}^2$ is extended to zero in $\left[ 0,  M \right] ^2 \setminus \Omega$. Integrating over $\Omega$ the first term of the sum in the right-hand side of \eqref{eq:aux01} we get
\begin{equation*}
\begin{split}
	\int_\Omega \left( \int_a^b \abs*{\partial_{xx} v_h(t,y)}^2 \,dt \right) \, dx \, dy &\leq \int_{0}^{M} \int_{0}^{M} \int_{0}^{M} \abs*{\partial_{xx} v_h(t,y)}^2 \, dt \, dx \, dy \\
	&= M \int_{0}^{M} \int_{0}^{M} \abs*{\partial_{xx} v_h(t,y)}^2 \, dt \, dy \\
	&= M \int_{\Omega} \abs*{\partial_{xx} v_h(t,y)}^2 \, dt \, dy.
\end{split}
\end{equation*}
In a similar way, integrating over $\Omega$ the last term of \eqref{eq:aux01}, we obtain
\begin{equation*}
	\int_\Omega \sum_{t_\ell \in I[a,b]} \abs*{\jump{\partial_x v_h}_{\gl}(t_\ell,y)}^2 \, dx \, dy \leq C \sum_{\ell \in \is} \int_{\gl} \jump{\partial_n v_h}_{\gl}^2  \, ds.
\end{equation*}
Hence we have
\begin{equation*}
	\int_{\Omega} \abs*{\partial_x v_h(x,y)}^2 \, dx \, dy \leq C \int_{\Omega} \abs*{\partial_{xx} v_h}^2 \, dx \, dy + C \sum_{\ell \in \is} \int_{\gl} \jump{\partial_n v_h}_{\gl}^2 \, ds.
\end{equation*} 
We focus on the estimate of the last integral. By the mortar condition~\eqref{eq:mortarkernel} the average value of $\jump{\partial_n v_h}_{\gl}$ over $\gl$ is zero. Thus the standard trace theorem and Poincaré inequality yield
\begin{equation*}
	\int_{\gl} \jump{\partial_n v_h}_{\gl}^2 ds \leq C_{m(\ell)} \abs*{v_h}^2_{H^2(\Omega_{m(\ell)})} + C_{s(\ell)} \abs*{v_h}^2_{H^2(\Omega_{s(\ell)})}.
\end{equation*}
Summing over all the interfaces we obtain~\eqref{eq:est1}.
With similar computations for the $y$-derivative, we can find a constant $C>0$ such that for every $v_h \in V_h$, it holds
\begin{equation}\label{eq:est_h1}
	\sum_{k \in \io} \abs*{v_h}^2_{H^1(\Omega_k)} \leq C\sum_{k \in \io} \abs{v_h}^2_{H^2(\Omega_k)}.
\end{equation}
Furthermore, observing that $V_h \subset H^1_0(\Omega)$, a standard Poincaré inequality yields
\begin{equation}\label{eq:est_l2}
	\sum_{k \in \io} \norm{v_h}^2_{L^2(\Omega_k)} \leq C\sum_{k \in \io} \abs{v_h}^2_{H^1(\Omega_k)}.
\end{equation}
Finally, the thesis follows by combining \eqref{eq:est_h1} and \eqref{eq:est_l2}.
\end{proof}
\end{lemma}
We recall that $\norm{\cdot}_X$ is defined by
\begin{equation*}
	\norm{v}_X^2 := \sum_{k \in \io} \norm{v}_{H^2(\Omega_k)}^2 + \sum_{\ell \in \is} \norm{\jump{\dn v}_{\gl}}_{H^{\nicefrac{1}{2}}(\gl)}^2.
\end{equation*}
\begin{lemma}\label{lemma:es1}
Let $s = \max (4,p+1)$. There exists a constant $C > 0$ such that, for all $v \in H^{s}(\Omega)$,
\begin{equation*}
	\inf_{v_h \in V_h} \norm{v - v_h}_X \leq C h^{p - 1} \norm{w}_{H^{s}(\Omega)}.
\end{equation*}
\end{lemma}
\begin{proof}
As $W_{\ell} \subset H^{\nicefrac{1}{2}}_{00}(\gl)$, every $w_h \in W_{\ell}$ can be extended to a function
$\tilde{w}_h \in H^{\nicefrac{1}{2}}(\partial\Omega_{s(\ell)})$. 
Let $\hh_{h,\ell} \tilde{w}_h \in X_{k,h}$ be such that $\abs{\hh_{h,\ell} \tilde{w}_h}_{H^2(\Omega_{s(\ell)})}=0$ and
fulfilling $\hh_{h,\ell} \tilde{w}_h \in H^1_0(\Omega_{s(\ell)})$ and $\partial_n \left( \hh_{h,\ell} \tilde{w}_h \right) = \tilde{w}_h$ on $\gl$, where we recall that $\textbf{n}$ on $\gl$ is the outer normal with respect to $\partial \Omega_{m(\ell)}$.
Then 
\begin{equation*}
	\norm{\hh_{h,\ell} \tilde{w}_h}_{H^2(\Omega_{s(\ell)})} \leq C \norm{\tilde{w}_h}_{H^{\nicefrac{1}{2}}(\partial \Omega_{s(\ell)})} \leq C \norm{w_h}_{H^{\nicefrac{1}{2}}(\gl)}.
\end{equation*}
We further extend $\hh_{h,\ell} \tilde{w}_h$ to $0$ outside $\Omega_{s(\ell)}$. Let $v \in H^{p+1}(\Omega)$ and let $\Pi_h v \in X_h$ be the global spline projection of $v$ in $X_h$, defined in Proposition~\ref{prop:globalproj}. We define an element $v_h \in V_h$ such that
\begin{equation*}
	v_h := \Pi_h v - \sum_{\ell \in \is} \hh_{h,\ell} \M_\ell \jump{\partial_n \Pi_h v}_{\gl}.
\end{equation*}
From the definition of $\Pi_h$ we have that, for all $\tau_h \in M_h$,
\begin{equation*}
	\int_{\gl}\jump{\dn v_h}\,\tau_h \, d\sigma = \int_{\gl} \left( \jump{\dn \Pi_h v} - \M_\ell \jump{\dn \Pi_h v} \right) \tau_h \, d\sigma = 0.
\end{equation*}
That is $v_h \in V_h$. Then, we can write
\begin{equation*}
	\norm{v - v_h}_X \leq \norm{v - \Pi_h v}_X + \norm*{\sum_{\ell \in \is} \hh_{h,\ell} \M_\ell \jump{\dn \Pi_h v}_{\gl}}_X.
\end{equation*}
The first term is estimated in Proposition~\ref{prop:globalproj}.
On the other hand, using the definition of $\hh_{h,\ell}$, we get
\begin{equation*}
\begin{split}
	\norm*{\sum_{\ell \in \is} \hh_{h,\ell} \M_\ell \jump{\dn \Pi_h v}_{\gl}}_X^2 &\leq \sum_{\ell \in \is} \norm*{\hh_{h,\ell} \M_\ell \jump{\dn \Pi_h v}_{\gl}}_{H^2\left( \Omega_{s(\ell)}\right) }^2 + \sum_{\ell \in \is} \norm*{\M_\ell \jump{\dn \Pi_h v}_{\gl}}_{H^{\nicefrac{1}{2}}(\gl)}^2 \\ &\leq C \sum_{\ell \in \is} \norm*{\M_\ell \jump{\dn \Pi_h v}_{\gl}}_{H^{\nicefrac{1}{2}}(\gl)}^2.
\end{split}
\end{equation*}
The $H^{\nicefrac{1}{2}}_{00}$-stability of the mortar projector $\M_\ell$, stated in Lemma~\ref{lemma:projproperties}, and Proposition~\ref{prop:globalproj} yield
\begin{equation*}
\begin{split}
	\norm*{\M_\ell \jump{\dn \Pi_h v}_{\gl}}_{H^{\nicefrac{1}{2}}(\gl)}^2 &\leq \norm*{\jump{\dn \Pi_h v}_{\gl}}_{H^{\nicefrac{1}{2}}(\gl)}^2 \\
	&\leq C h^{2(p-1)} \left(\norm*{v}^2_{H^{s}\left( \Omega_{m(\ell)}\right) } + \norm*{v}^2_{H^{s}\left( \Omega_{s(\ell)}\right) } \right). 
\end{split}
\end{equation*}
Thanks to Assumption~\ref{ass:quasiunif}, summing over the interfaces we obtain the thesis.
\end{proof}


